Studying LLM Performance on Closed- and Open-source Data

Large Language models (LLMs) are finding wide use in software engineering practice. These models are extremely data-hungry, and are largely trained on open-source (OSS) code distributed with permissive licenses. In terms of actual use however, a great deal of software development still occurs in the for-profit/proprietary sphere, where the code under development is not, and never has been, in the public domain; thus, many developers, do their work, and use LLMs, in settings where the models may not be as familiar with the code under development. In such settings, do LLMs work as well as they do for OSS code? If not, what are the differences? When performance differs, what are the possible causes, and are there work-arounds? In this paper, we examine this issue using proprietary, closed-source software data from Microsoft, where most proprietary code is in C# and C++. We find that performance for C# changes little from OSS --> proprietary code, but does significantly reduce for C++; we find that this difference is attributable to differences in identifiers. We also find that some performance degradation, in some cases, can be ameliorated efficiently by in-context learning.

==> limitations.tex <==
\section{Limitations[Prem \& Chris]}



In our study, the evaluation of LLMs' generalization performance is confined primarily to two programming languages: C\# and C++. 
This focus, while providing in-depth insights for these specific languages, presents a limitation in terms of the generalizability of our findings across the spectrum programming languages.
Different programming languages have unique syntaxes, idioms, and use-cases~\cite{allamanis2018survey} and the performance of LLMs in one language may not directly translate to another. 
This limitation is particularly relevant when considering languages with different paradigms (e.g., functional vs. object-oriented) or usage domains (e.g., web development vs. system programming). 
However, our choice to focus on C\# and C++ is still valid in certain contexts. 
Both languages are widely used in industry and academia, making our findings relevant to a significant portion of the software development community~\cite{meyerovich2013empirical}. 
Additionally, C\# and C++ offer a balance between modern, high-level programming features and low-level control, making them representative of a broad range of programming challenges and scenarios. 
Therefore, while our study's language scope is a limitation,, we claim that it still provides valuable insights into the generalization capabilities of LLMs within the context of programming languages in broad use both in OSS and commercial development.

Our study's reliance on pre-trained models such as CodeBERT presents a limitation. 
While these models are pivotal in understanding code through natural language processing, they may not fully represent the capabilities and limitations of newer or alternative LLM architectures.
Therefore, these findings may not hold for all models as technology advances in the field of LLMs for code.

%Additionally, the lack of access to the training data prevents us from studying the model's generalization or memorization through de-duplication processes.
Lack of access to the models' training data significantly limits our ability to investigate the models' generalization and memorization capabilities.
The question of how much of what a model generates is the result of memorized code snippets and how much is the result of generalization is a key question in evaluating the utility of such models.
